Data Driven Prediction Architecture for Autonomous Driving and its Application on Apollo Platform

Autonomous Driving vehicles (ADV) are on road with large scales. For safe and efficient operations, ADVs must be able to predict the future states and iterative with road entities in complex, real-world driving scenarios. How to migrate a well-trained prediction model from one geo-fenced area to another is essential in scaling the ADV operation and is difficult most of the time since the terrains, traffic rules, entities distributions, driving/walking patterns would be largely different in different geo-fenced operation areas. In this paper, we introduce a highly automated learning-based prediction model pipeline, which has been deployed on Baidu Apollo self-driving platform, to support different prediction learning sub-modules' data annotation, feature extraction, model training/tuning and deployment. This pipeline is completely automatic without any human intervention and shows an up to 400\% efficiency increase in parameter tuning, when deployed at scale in different scenarios across nations.

==> sections/_inactive_autotuning.tex <==
\section{Post Trajectory Generation}
\label{sec:post_trajectory_generation}

This section introduces a data-driven, learning-based method to tune the parameters in trajectory generation stage in the prediction module. This method takes the predicted paths with their probabilities from the deep learning models as priors, then for each path, we sample some candidate predicted trajectories based on different speed profiles. We assign the cost values for all candidate trajectories and compute the likelihood of the associated path using the smallest cost value. The candidate trajectory with that smallest cost value is the predicted trajectory in its associated path. The posterior of each path with its predicted trajectory is computed by the prior and likelihood. The cost of each candidate trajectory is computed by the weighted sum of three cost functions. We applied Siamese network to tune the weights by real-world road test data. The follow subsections introduce the details of the method.

\subsection{Prior}
\label{subsec:prior}
In Apollo, we have several deep learning behavior prediction models. One predicts lane sequences the target obstacle will go. Another predicts the intersection exits for the vehicles running within the area of an intersection. Both of the two models have the same format of the output which is the possible future paths with their probabilities. As shown in Figure \ref{fig:autotuning_example}(a), the red vehicle is the target vehicle that we want to make prediction and the blue vehicle is the autonomous driving ego vehicle. The deep learning behavioral model outputs three possible paths with their probabilities as the three red arrows. Their probabilities are 0.2, 0.4, 0.4 for turning right, going straight, and turning left, respectively. For each path, its probability from the deep learning behavioral model is used as prior in this poster processing method.

\begin{figure}
  \centering
  \includegraphics[width=8cm, height=8cm]{images/autotuning_example.png}
  \caption{The procedure of trajectory posterior processing.}
  \label{fig:autotuning_example}
\end{figure}


\subsection{Sampling}
\label{subsec:sampling}
To get the candidate trajectories with different speed profile, we sample multiple values of accelerations, and generate trajectories according to the sampled accelerations by constant acceleration movement. For each sampled trajectory, it goes along the central curve of the associated path. Figure \ref{fig:autotuning_example}(b) illustrates the sampling process.


\subsection{Cost Functions}
\label{subsec:cost_functions}
For each candidate trajectory, we designed three cost functions related to longitudinal acceleration, centripetal acceleration, and collision with ego vehicle. They represent longitudinal comfort, lateral comfort, and safety. The formula of these three cost functions are shown in Eq\eqref{cost:acc} to Eq\eqref{cost:collision}.

\begin{eqnarray}
     C_{acc} &=& \sum\limits_{i}a_i^2 \label{cost:acc} \\
     C_{centripetal\_acc} &=& \frac{1}{z_1}\sum\limits_{i}(v_i^2\kappa_i)^2 \label{cost:centripetal_acc} \\
     C_{collision} &=& \frac{1}{z_2}\sum\limits_{i}d_i^2 \label{cost:collision}
\end{eqnarray}
where $z_1$ and $z_2$ are the normalization terms. $d_i$ in Eq\eqref{cost:collision} is the distance between the the predicted trajectory point and the ego vehicle at the timestamp of the $i$th predicted trajectory point.

The total cost of a candidate trajectory as shown in Eq\eqref{cost:total} can be computed by the weighted sum of Eq\eqref{cost:acc}, Eq\eqref{cost:centripetal_acc}, and Eq\eqref{cost:collision}.
\begin{equation}
    C = w_1 C_{acc} + w_2 C_{centripetal\_acc} + w_3 C_{collision}
    \label{cost:total}
\end{equation}
where, $w_1$, $w_2$ and $w_3$ are the weights. In subsection \ref{subsec:siamese_network} we will discuss more about how to tune the weights automatically by data.

\subsection{Likelihood}
\label{subsec:likelihood}
The likelihood of a candidate trajectory can be computed by Eq
\begin{equation}
    \textrm{likelihood} = \exp(-C)
    \label{eq:likelihood}
\end{equation}
where $C$ is the total cost described in Eq\eqref{cost:total}, which designed to make the lower-cost candidate trajectories have higher likelihood probability.

With the likelihood computed by Eq\eqref{cost:total}, we can get the posterior probability by Eq\eqref{eq:posterior}.
\begin{equation}
    \textrm{Posterior} = \frac{1}{Z} \cdot \textrm{prior} \cdot \textrm{likelihood}
    \label{eq:posterior}
\end{equation}
where $Z$ is the normalization term to make the posteriors' sum of an obstacle to be one. As the example shown in Figure \ref{fig:autotuning_example}(d), the posterior probabilities are computed to correct the prior probabilities based on the likelihood involving comfort and safety.

\subsection{Siamese Network}
\label{subsec:siamese_network}
In this subsection, we introduce the method that is used to tune the weights. The assumption of the model is that the ground truth real trajectories are the optimal ones that have the least cost values. And we try to tune the weights to make the minimal cost of the sampled candidate trajectories close to the cost value of the ground truth trajectory.

We use $\xi$ to denote a sampled candidate trajectory, and $\hat\xi$ to denote a ground-truth real trajectory. We re-represent the cost function of as $C(\theta;\xi)$ and $C(\theta;\hat\xi)$. The objective function is designed as Eq\eqref{eq:objective}.
\begin{equation}
    L = \sum\limits_{j=0}^{N}\sum\limits_{i=0}^M|C(\theta;\hat\xi_i)-C(\theta;\xi_j) + \delta|_+
    \label{eq:objective}
\end{equation}
where, $|\cdot|_+$ is the maximum between $\cdot$ and 0, $N$ is the number of data (an obstacle at a timestamp), $M$ is the number of sample candidate trajectories for each data. $\delta$ is marginal factor which is a small positive constant. We tried to solve the optimization problem to minimize the objective function defined in Eq\eqref{eq:objective}. The marginal constant $\delta$ is necessary to avoid getting the solution that all weights are zero. On the other hand, it can filter out the sampled candidate trajectories whose cost values are much different from the ground-truth real trajectory's cost.

To solve the optimization defined in Eq\eqref{eq:objective}, we apply a Neural network shown in Figure \ref{fig:siamese}. The input layer consists of three cost differences and $delta$. It is followed by a ReLU activation function. The labels are all zero. We trained this model on the real-world road test data and apply the trained weights $w_1$, $w_2$, $w_3$ in the cost function.

This autotuning mechanism can learn the weights according to the local driving behavior, avoiding manual parameters tuning and more fit to the traffic in a specific area.


\begin{figure*}
  \centering
  \includegraphics[width=12cm, height=4.8cm]{images/siamese.png}
  \caption{Siamese network for autotuning.}
  \label{fig:siamese}
\end{figure*}



==> sections/_inactive_offline_architecture.tex <==
\section{Offboard Architecture}
\label{sec:offline_architecture}
In this section, we introduce the architecture to process data and model training offline. It consists of five data processing applications including 1) automatic data annotation, 2) feature extraction, 3) model training, 4) auto tuning, and 5) results evaluation. The whole workflow and the relationship among the five data applications are described in Figure \ref{fig:offline_architecture}.

\subsection{Automatic Data Annotation}
\label{subsec:data_labeling}
Data labeling takes the obstacle information sequence data from Database 1.

\subsection{Feature Extraction}
\label{subsec:feature_extraction}


\subsection{Model Training}
\label{subsec:model_training}


\subsection{Auto Tuning}
\label{subsec:auto_tuning}


\subsection{Results Evaluation}
\label{subsec:result_evaluation}


\begin{figure*}
  \centering
  \includegraphics[width=14cm, height=9cm]{images/offline_architecture.png}
  \caption{Offline Architecture of the prediction module on Apollo autonomous driving open-source platform.}
  \label{fig:offline_architecture}
\end{figure*}


==> sections/_inactive_problem_statement.tex <==
\section{Problem Statement}
\label{sec:problem_statement}
For an autonomous driving vehicle, it is important to make correct prediction of its surrounding obstacles' future movements especially the surrounding vehicles in urban drive scenarios.More precise prediction is helpful for making more appropriate decisions to reduce the risk of collisions and improve the comfort level.

To solve this problem, we are given the historical states and surrounding environment for each vehicle. A state includes position, velocity, heading, and shape. The surrounding environment includes lanes, road boundaries, intersections, crosswalks and nearby dynamic obstacles. The prediction model output a predicted trajectory with a sequence of positions representing its future movement.




==> sections/_inactive_related_works.tex <==
\section{Related Works}
\label{sec:related_works}
